Counterfactual Image Generation for adversarially robust and interpretable Classifiers

Neural Image Classifiers are effective but inherently hard to interpret and susceptible to adversarial attacks. Solutions to both problems exist, among others, in the form of counterfactual examples generation to enhance explainability or adversarially augment training datasets for improved robustness. However, existing methods exclusively address only one of the issues. We propose a unified framework leveraging image-to-image translation Generative Adversarial Networks (GANs) to produce counterfactual samples that highlight salient regions for interpretability and act as adversarial samples to augment the dataset for more robustness. This is achieved by combining the classifier and discriminator into a single model that attributes real images to their respective classes and flags generated images as "fake". We assess the method's effectiveness by evaluating (i) the produced explainability masks on a semantic segmentation task for concrete cracks and (ii) the model's resilience against the Projected Gradient Descent (PGD) attack on a fruit defects detection problem. Our produced saliency maps are highly descriptive, achieving competitive IoU values compared to classical segmentation models despite being trained exclusively on classification labels. Furthermore, the model exhibits improved robustness to adversarial attacks, and we show how the discriminator's "fakeness" value serves as an uncertainty measure of the predictions.

==> literature.tex <==


% NN prone to artifacts
Deep neural networks are easily fooled (2015)
Adversarial examples in the physical world (2016)

% advsersarial robustness
"Learn2Perturb: an End-to-end Feature Perturbation Learning to Improve Adversarial Robustness" 2020
adds learnable noise distributions to the outputs of a neural network models at various feature levels.

% intrinsic explanations
Learning Deep Features for Discriminative Localization
https://arxiv.org/abs/1512.04150
Understanding Deep Image Representations by Inverting Them (2014)
Inverting CNNs for feature visualisation
Understanding deep image representations by inverting them (2015)


% post'hoc explanations
% surrogate based
LIME
https://arxiv.org/abs/1602.04938
LIME is a
generalized method suitable for both image and non-image
inputs that boils down to set theory: if part of the input were
masked, would the overall classification get better or worse?
By noting which parts of the input make the most significant
difference, the LIME algorithm derives a linear classifier which
approximates the non-linear NN, and the linear, approximating
classifier is then used to produce a mask for the input that
highlights salient regions
% gradient based
GradCAM
https://arxiv.org/abs/1610.02391
GradCAM algorithm harnesses backpropagation directly to derive
an expression for localizing the most salient regions [4]. Its
innovation came from measuring image region contribution at
a layer closer to the classifying end of the NN than the input
GradCAM++
https://arxiv.org/abs/1710.11063
Score-CAM: Scoreweighted visual explanations for convolutional neural networks
https://arxiv.org/abs/1910.01279
Ablation-CAM: Visual explanations for deep convolutional network via
gradient-free localization
https://openaccess.thecvf.com/content_WACV_2020/papers/Desai_Ablation-CAM_Visual_Explanations_for_Deep_Convolutional_Network_via_Gradient-free_Localization_WACV_2020_paper.pdf
Visualizing and understanding convolutional network
https://arxiv.org/abs/1311.2901
Interpretable and finegrained visual explanations for convolutional neural networks
https://arxiv.org/abs/1908.02686

Counterfactual Image Enhancement for Explanation of Face Swap Deepfakes (2022)
https://link.springer.com/chapter/10.1007/978-3-031-18910-4_40#Sec2
Targeted attack on images using a classifier trained for detecting deepfakes. The gradient updates are supposed to highlight features that give away the deepfakes. 


% perturbation based
RISE: Randomized Input Sampling for Explanation of Black-box Models
https://arxiv.org/abs/1806.07421
Understanding deep networks via extremal perturbations and
smooth masks
https://arxiv.org/abs/1910.08485

"EXPLAINING IMAGE CLASSIFIERS BY
COUNTERFACTUAL GENERATION" (2019)
samples masks for obscuring parts of the image which are then in-filled using a pretrained in-filling model.

% combined gradient + perturbation based
Visual Explanation by Unifying Adversarial
Generation and Feature Importance Attributions (2021)
combines gradient based and perturbation based explanations.

%adversarial attacks
Intriguing properties of neural networks (2013)
First work on imperceptible perturbations that drastically change a networks prediction.

EXPLAINING AND HARNESSING ADVERSARIAL EXAMPLES
https://arxiv.org/abs/1412.6572

% adversarial explanations
“Robustness may be at odds with accuracy" (2018)
 demonstrated that non-minimal adversarial examples contained salient features
when networks were adversarially trained. Here, non-minimal
means adversarial examples which have not been optimized
for minimal perturbation distance, but only for maximal loss
on the objective function.

"Adversarial Explanations for Understanding Image
Classification Decisions and Improved Neural
Network Robustness" (2019)
create adversarial perturbations of images subject to a lipschitz constraint which improves the classifier's robustness and creates adversarial examples with very discernible features for non-linear explanation mechanism (as opposed to gradcam or LIME)

"Generating Adversarial Examples in One Shot
With Image-to-Image Translation GAN" (2019)
image-to-image translation using a gan with 3 discriminators.

"EXPLAINING IMAGE CLASSIFIERS BY
COUNTERFACTUAL GENERATION" (2019)


"Combining Similarity and Adversarial Learning to
Generate Visual Explanation:
Application to Medical Image Classification" (2020)
Uses two generators to explain predictions of a classifier (which is not retrained). One generator is in charge of generating counterfactual images, while the other reconstructs the original image as closely as possible. The authors reason that comparing the original image with its
generated adversarial sample exposes the method to a risk of
reconstruction error. Some details of the original image can be absent from the generated adversarial sample. However these
details are not discriminative for the classifier in the sense
that their sole presence would not change the classification
score. We argue that the reason for this is the fact that the classifier is not retrained and that it has no way of telling real and fake images apart. This motivates our use of a single, retrained classifier with 3 outputs.

"Scientific Discovery by Generating
Counterfactuals using Image Translation" (2020)
Use cycleGAN (with two discriminators) for translating from one class to another and retrain a classifier to validate that the class has really changed. However, the generator and classifier trainings are decoupled, meaning that there are no gradients flowing from the classifier to the generator. so the robustness gained from adversarial training is lost.


Learning What Makes a Difference
from Counterfactual Examples and
Gradient Supervision (2020)
https://arxiv.org/abs/2004.09034
look for minimally different samples in the dataset with different classes

Degenerative adversarial neuroimage nets for brain scan simulations: Application in ageing and dementia (2022)
Uses conditional generative image-to-image models applied to Brain MRI for visualizing the process of ageing and dementia. However, the discriminators do not receive the conditions as input. Therefore the extent to which the generator respects the conditioning is questionable. 

Leveraging conditional generative models in a general explanation framework of classifier decisions (2022)
https://www.sciencedirect.com/science/article/pii/S0167739X22000632?fr=RR-2&ref=pdf_download&rr=7fc448d4491c41b1#b43
Very similar in that they use a gan for creating counterfactural examples that fool a classifier and a discriminator. However, their classifier is pre-trained and not updated anymore. Furthermore, they use two distinct generators for mapping from one domain to the other, instead of a single one. They also use cycle-consistency, but they enforce an L1 and L2 distance between the original image and the cycled image, which would imply the model to add and remove the exact same damage - not what we want.


